Learning Performance-Oriented Control Barrier Functions Under Complex Safety Constraints and Limited Actuation

Control Barrier Functions (CBFs) provide an elegant framework for constraining nonlinear control system dynamics to remain within an invariant subset of a designated safe set. However, identifying a CBF that balances performance-by maximizing the control invariant set-and accommodates complex safety constraints, especially in systems with high relative degree and actuation limits, poses a significant challenge. In this work, we introduce a novel self-supervised learning framework to comprehensively address these challenges. Our method begins with a Boolean composition of multiple state constraints that define the safe set. We first construct a smooth function whose zero superlevel set forms an inner approximation of this safe set. This function is then combined with a smooth neural network to parameterize the CBF candidate. To train the CBF and maximize the volume of the resulting control invariant set, we design a physics-informed loss function based on a Hamilton-Jacobi Partial Differential Equation (PDE). We validate the efficacy of our approach on a 2D double integrator (DI) system and a 7D fixed-wing aircraft system (F16).

==> secs/hocbf.tex <==
\section{Construction of High-Order CBF}
\label{sec:hocbf}
\begin{definition}[Class $\mathcal{K}$ function]
A continuous function $\alpha(\cdot):[0, a) \mapsto [0, \infty)$ belongs to class $\mathcal{K}$ if it satisfies $\alpha(0) = 0$ and strictly increasing. 
\end{definition}

\begin{definition}[Relative degree]
A (sufficiently many times) differentiable function $b:\mathbb{R}^n \mapsto \mathbb{R}$ has a relative degree $m$ with respect to system~\eqref{eq:dynamics} if $b$ has to be differentiated $m$ times along the system dynamics before the control input $u$ explicitly shows for all states $x$ in the corresponding derivative. 
\end{definition}

For a function $b(x):\mathbb{R}^n \mapsto \mathbb{R}$ with relative degree $m$, we define a sequence of functions $\psi_i(x):\mathbb{R}^n \mapsto \mathbb{R}, i=0, 1, \cdots, m$ as
\begin{equation}
\begin{aligned}
    \psi_0(x) & = b(x), \\
    \psi_i(x) & = \dot{\psi}_{i-1}(x) + \alpha_i(\psi_{i-1}(x)), i = 1, \cdots, m, 
\end{aligned}
\end{equation}
where $\alpha_i$ denotes the $(m-i)$-th order differentiable class $\mathcal{K}$ function. Consequently, we define the following sets associated with each $\psi_i(x)$:
\begin{equation} \label{eq:D_i}
    \mathcal{D}_i = \{x \mid \psi_{i-1}(x) \geq 0 \}, i = 1, \cdots, m. 
\end{equation}

\begin{definition}[High-order control barrier function]
\label{def:HOCBF}
A function $b(\cdot):\mathbb{R}^n \mapsto \mathbb{R}$ is a high-order control barrier function of relative degree $m$ for system~\eqref{eq:dynamics} if there exists $(m-i)$-th order differentiable class $\mathcal{K}$ functions $\alpha_i$ for $i=1, \cdots, m-1$ such that 
\begin{equation}
    \underset{u\in \mathcal{U}}{\sup} \left [ L^m_f b(x) + (L_g L_f^{m-1}b(x))u + O(b(x)) + \alpha_m(\psi_{m-1}(x)) \right] \geq 0,
\end{equation}
for all $x \in \cap_{i=1}^{m-1} \mathcal{D}_i$ where 
\begin{equation*}
    O(b(x)) = \sum_{i=1}^{m-1} L_f^i(\alpha_{m-i} \circ \psi_{m-i-1})(x),
\end{equation*} 
$L_f^m$ denotes the Lie derivative along $f$ for $m$ times, and $L_g$ denotes the Lie derivative along $g$. In addition, $b(x)$ satisfies $L_g L_f^{m-1}b(x) \neq 0$ on the boundary of $\cap_{i=1}^{m-1} \mathcal{D}_i$.
\end{definition}

Given a HOCBF, we define the associated safe control set as
\begin{equation}
    K_{hocbf} = \left \{ u \in \mathcal{U} \mid  \left [ L^m_f b(x) + (L_g L_f^{m-1}b(x))u + O(b(x)) + \alpha_m(\psi_{m-1}(x)) \right] \geq 0 \right \}
\end{equation}

\begin{theorem}[\cite{xiao2019control}]
Given a HOCBF defined in Definition~\ref{def:HOCBF}. If $x(0) \in \cap_{i=1}^{m-1} \mathcal{D}_i$, then any Lipschitz continuous controller $u(x) \in K_{hocbf}(x)$ renders the set $\cap_{i=1}^{m-1} \mathcal{D}_i$ forward invariant. 
\end{theorem}

We propose to first formulate $b(x)$ as a composite CBF using the formulation from Section~\ref{sec:composite_CBF}, which by construction guarantees that $\cap_{i=1}^{m-1} \mathcal{D}_i$ does not intersect any unsafe region. Next, we parameterize $\alpha_{1:m}$ as NNs that belong to class $\mathcal{K}$ by construction. 

\subsection{Parameterization of class $\mathcal{K}$ functions}
We propose a NN parameterization of class $\mathcal{K}$ functions based on the constrained monotonic NNs that are shown to be universal approximators of continuous monotone functions~\cite{runje2023constrained}. We first illustrate the parameterization of the constrained monotonic NNs below. 

Let $y\in\mathbb{R}$ be a scalar input~\footnote{Since the class $\mathcal{K}$ function $\alpha(y)$ is a univariate function, we only consider a scalar input here for simplicity. We refer the readers to~\citet{runje2023constrained} for the multivariate setting. } and $\breve{\rho}:\mathbb{R}\mapsto \mathbb{R}$ be a smooth, zero-centered, increasing, convex, lower-bounded functions such as SELU and ELU. Then, we define
\begin{equation*}
    \hat{\rho}(y) = - \breve{\rho}(-y), \quad \tilde{\rho}(y) = 
    \begin{cases}
        \breve{\rho}(y+1) - \breve{\rho}(1) & \text{if } y < 0, \\
        \hat{\rho}(y-1) + \breve{\rho}(1) & \text{otherwise}. 
    \end{cases}
\end{equation*}
As shown in Fig.~\ref{}, $\hat{\rho}$ is a concave, upper-bounded function and $\tilde{\rho}$ is a bounded function. Consider a vector input $z \in \mathbb{R}^k$ and an activation function $\rho:\mathbb{R}^k \mapsto \mathbb{R}^k$ defined by
\begin{equation}
    \rho(z)[i] = \begin{cases}
       \breve{\rho}(z[i]), &  \text{if } 1 \leq i \leq \breve{s}, \\
      \hat{\rho}(z[i]),    & \text{if } \breve{s} < i \leq \breve{s} + \hat{s}, \\
      \tilde{\rho}(z[i]), &  \text{if }, \breve{s} + \hat{s} < i \leq \breve{s} + \hat{s} + \tilde{s},
    \end{cases}
\end{equation}
where $z[i]$ denotes the $i$-th entry of $z$, and $(\breve{s}, \hat{s}, \tilde{s})$ are non-negative integers satisfying $\breve{s} + \hat{s} + \tilde{s} = k$. Then, we parameterize a constrained monotonic NN as:
\begin{equation} \label{eq:nn_alpha_1}
    \begin{aligned}
       \bar{\alpha}(y) &= W^+_L\rho(W^+_{L-1}\rho( \cdots \rho(W^+_0 y + b_0) \cdots ) + b_{L-1}) + b_L, \\
    \end{aligned}
\end{equation}
where $W^+_{0:L}$ are positive linear weights and $b_{0:L}$ are unconstrained biases. It can be easily verified that $\bar{\alpha}(y)$ is a strictly increasing function. By applying different types of activations (convex, concave, and bounded) on different entries, $\rho(\cdot)$ improves the expressivity of $\bar{\alpha}(y)$ such that it is not necessarily a convex function even though only positive linear weights are applied. Finally, we parameterize the NN class $\mathcal{K}$ function as 
\begin{equation} \label{eq:nn_alpha_2}
    \alpha(y) = \bar{\alpha}(y) - \bar{\alpha}(0),
\end{equation}
to ensure $\alpha(0) = 0$. In our experiments, we choose $\breve{\rho}$ as \textcolor{blue}{xxx} function and parameterize each $\alpha_i$ in the HOCBF as~\eqref{eq:nn_alpha_1} and~\eqref{eq:nn_alpha_2} with $(W^+_{0:L}, b_{0:L})$ being the training parameters. The indices $(\breve{s}, \hat{s}, \tilde{s})$ for an activation layer with input dimension $k$ are fixed as $\breve{s} = \lfloor 0.4k \rfloor, \hat{s} = \lfloor 0.4k \rfloor, \tilde{s} = k - \breve{s} - \hat{s}$ where $\lfloor \cdot \rfloor$ denotes the round down function to the nearest integer. 

==> secs/train_hocbf.tex <==

\section{Training of Composite HOCBF}
Assuming the class $K$ functions in the HOCBF are parameterized by $\alpha_i(x; \theta_{\alpha, i})$ and the composite CBF is parameterized by $b(x; \theta_b)$. Following the definition of HOCBF, the safe invariant set is given by $\mathcal{D}:=\cup_{i=1}^m \mathcal{D}_i$ and the safe control set $K_{hocbf}(x)$. We want to learn a composite HOCBF such that the volume of the safe invariant set $\mathcal{D}$ is enlarged (tightness objective) and for states in $\mathcal{D}$, the safe control set $K_{hocbf}(x)$ is non-empty (feasibility objective). 

\subsection{Tightness Objective}
Since $\mathcal{D}= \cap_{i=1}^m \mathcal{D}_i$ is given by the intersection of $m$ sets $\mathcal{D}_i$ defined in~\eqref{eq:D_i}, following Section~\ref{sec:composite_CBF}, we can define a smooth lower bound $\underline{h}(x)$ such that $\{x \mid \underline{h}(x) \geq 0\} \Rightarrow x \in \mathcal{D}$. Then, we can enlarge $\mathcal{D}$ by optimizing the following objective
\begin{equation}  \label{eq:tightness_obj}
    \underset{\theta}{\text{minimize}} \quad \frac{1}{N} \sum_{i=1}^N \text{ReLU}(-\underline{h}(x_i;\theta)),
\end{equation}
where $\{x_i\}_{i=1}^N$ are sampled states from the domain $\mathcal{X}$ in the state space. The above objective encourages the inner approximation of the safe forward invariant set to include as many states as possible in $\mathcal{X}$. One important feature of the learning objective~\eqref{eq:tightness_obj} is that unlike~\cite{}, it does not require distinguishing safe and unsafe samples which significantly simplifies the learning process. 

\subsection{Feasibility Objective}
Let $\{v_i\}_{i=1}^{N_u}$ denote the $N_u$ vertices of the polyhedral set of admissible control inputs $\mathcal{U}$. At a given state $x$, the safe control set $K_{hocbf}$ is non-empty if and only if 
\begin{equation}
 \exists v_i \text{ s.t. }  L^m_f b(x) + O(b(x)) + \alpha_m(\psi_{m-1}(x)) \geq - (L_g L_f^{m-1}b(x)) v_i. 
\end{equation}
Define $\mathcal{V}_i := \{x \mid L^m_f b(x) + O(b(x)) + \alpha_m(\psi_{m-1}(x)) \geq - (L_g L_f^{m-1}b(x)) v_i \}$. We have the set of states where $K_{hocbf}(x)$ is non-empty is given by $\mathcal{F}: = \cup_{i=1}^{N_u} \mathcal{V}_i$. Similarly, we can derive a single smooth function $\underline{\nu}(x)$ such that $\{x \mid \underline{\nu}(x) \geq 0\} \subseteq \cup_{i=1}^{N_u} \mathcal{V}_i.$ To promote feasibility, we want the superlevel set $\{x \mid \underline{\nu}(x) \geq 0\}$ to cover as many states as possible. 


\begin{align}
    \min_{\theta,\beta} \mathbb{E}_{x \sim \rho} [\max(-L_fh(x) - L_gh(x) u^\star(x)- \alpha(h(x)),0)] - \lambda_1 \mathbb{E}_{x \sim \rho} [\alpha(h(x))]+ \lambda_2 \|\beta\|_2 \\
    %
     \max_{\theta,\beta} \mathbb{E}_{x \sim \rho} [L_fh(x) + L_gh(x) u^\star(x)+ \alpha(h(x))] - \lambda_2 \|\beta\|_2 
\end{align}

\subsection{Inferece constraint}
To avoid conflicting objectives, we want to enforce the following constraints during training
\begin{equation}
    \underline{h}(x) \geq 0 \Rightarrow \underline{\nu}(x) \geq 0. 
\end{equation}
Note that $A \Rightarrow B \Leftrightarrow \neg A \vee B$. Then we can find a single smooth function $\underline{\mu}(x)$ such that 
\begin{equation}
    \{ x \mid \underline{\mu}(x) \geq 0 \} \subseteq \{x \mid \underline{h}(x) \geq 0 \Rightarrow \underline{\nu}(x) \geq 0\}.
\end{equation}
The final learning objective is given by 
\begin{equation}  \label{eq:tightness_obj}
    \underset{\theta}{\text{minimize}} \quad \frac{1}{N} \sum_{i=1}^N (\text{ReLU}(-\underline{h}(x_i;\theta)) + \lambda \text{ReLU}(-\underline{\mu}(x_i;\theta))) 
\end{equation}

\subsection{Comparison with existing training methods}
Elaborate on what our method reduces to and compare it with the existing CBF learning formulations. 


